SAFER-Splat: A Control Barrier Function for Safe Navigation with Online Gaussian Splatting Maps

SAFER-Splat (Simultaneous Action Filtering and Environment Reconstruction) is a real-time, scalable, and minimally invasive action filter, based on control barrier functions, for safe robotic navigation in a detailed map constructed at runtime using Gaussian Splatting (GSplat). We propose a novel Control Barrier Function (CBF) that not only induces safety with respect to all Gaussian primitives in the scene, but when synthesized into a controller, is capable of processing hundreds of thousands of Gaussians while maintaining a minimal memory footprint and operating at 15 Hz during online Splat training. Of the total compute time, a small fraction of it consumes GPU resources, enabling uninterrupted training. The safety layer is minimally invasive, correcting robot actions only when they are unsafe. To showcase the safety filter, we also introduce SplatBridge, an open-source software package built with ROS for real-time GSplat mapping for robots. We demonstrate the safety and robustness of our pipeline first in simulation, where our method is 20-50x faster, safer, and less conservative than competing methods based on neural radiance fields. Further, we demonstrate simultaneous GSplat mapping and safety filtering on a drone hardware platform using only on-board perception. We verify that under teleoperation a human pilot cannot invoke a collision. Our videos and codebase can be found at https://chengine.github.io/safer-splat.

==> sections/limitations_future_work.tex <==
\section{Limitations and Future Work}
\label{sec:limitations_future_work}
SAFER-Splat assumes that the underlying GSplat map is relatively accurate with respect to the real-world, which does not hold in some situations, especially with dynamic objects.
Future work will seek to improve SAFER-Splat in these cases by accounting for dynamic objects in an uncertainty-aware optimization framework. Second, we hope to expand SAFER-Splat beyond double-integrator systems, e.g., contact-rich dynamical systems. Next, SAFER-Splat can be deployed on lower-end hardware as GSplat maps become more lightweight \cite{shorinwa2024fast}. Furthermore, SplatBridge can be made more robust to inaccurate camera pose estimates, which  affects the accuracy of the GSplat. Finally, we seek to extend SAFER-Splat to semantic multi-robot mapping \cite{yu2025hammer, shorinwa2025siren}, semantic-aware safety, and simultaneous deployment with high-level planners like Vision-Language-Action (VLA) models. 

==> sections/reconstruction.tex <==
\section{Real-time 3D Reconstruction}
\label{sec:reconstruction}

\subsection{Hardware}
We execute our pipeline on a small drone platform. The Starling 2 is a 220 mm drone, equipped with a suite of sensors, yielding fisheye RGB images and time-of-flight point clouds. The platform also maintains a pose estimate through visual inertial odometry (VIO) and can track position, velocity, and acceleration commands with a low-level PX4 controller. The camera images, point clouds, and VIO poses are sent through ROS2 \cite{macenski2022robot} to an off-board desktop computer (RTX 4090) via a WiFi connection. The desktop computer then sends accelerations back to the drone. A joystick is used for the operator to send high-level control actions to the safety layer. SAFER-Splat's ROS nodes are made available in our codebase. 

\subsection{SplatBridge}
The incoming stream of RGB images, time-of-flight point clouds, and estimated poses are used to train a Gaussian Splat in real-time. We utilize an extension of NerfBridge \cite{yu2023nerfbridge}, called SplatBridge, to interface with the Gaussian Splatting implementation in Nerfstudio \cite{nerfstudio}. At every keyframe, SplatBridge loads the image into a running buffer and seeds Gaussians from the point cloud. Asynchronous to the stream, SplatBridge optimizes the Gaussian attributes and the camera poses initialized at the VIO estimates, minimizing the loss proposed by \cite{kerbl3Dgaussians}. The safety layer maintains a reference to the Gaussian attributes maintained by SplatBridge. 
